Optimizing Information Credibility in Social Swarming Applications

With the advent of smartphone technology, it has become possible to conceive of entirely new classes of applications. Social swarming, in which users armed with smartphones are directed by a central director to report on events in the physical world, has several real-world applications: search and rescue, coordinated fire-fighting, and the DARPA balloon hunt challenge. In this paper, we focus on the following problem: how does the director optimize the selection of reporters to deliver credible corroborating information about an event. We first propose a model, based on common intuitions of believability, about the credibility of information. We then cast the problem posed above as a discrete optimization problem, and introduce optimal centralized solutions and an approximate solution amenable to decentralized implementation whose performance is about 20% off on average from the optimal (on real-world datasets derived from Google News) while being 3 orders of magnitude more computationally efficient. More interesting, a time-averaged version of the problem is amenable to a novel stochastic utility optimization formulation, and can be solved optimally, while in some cases yielding decentralized solutions. To our knowledge, we are the first to propose and explore the problem of extracting credible information from a network of smartphones.

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\subsection{Methodology}
\begin{figure}[!t]
\centering
\includegraphics[width=3in]{pics/news.eps}
\caption{An example of Google News} \label{fig:news}
\end{figure}
In this section, we try to evaluate our credibility framework by
using Google News. As shown in Fig. \ref{fig:news}, when we search a
specific event, like ``House passes health care reform
bill\footnote{The House of Representatives on March 21 (ET) passed a
sweeping \$940 billion health care bill in a historic vote that will
dramatically change the U.S. health care system.}" in Google News,
the server returns several results. Because each result has a
corresponding provenance (e.g., ``Martinsville Bulletin", ``Vanity
Fair", and ``Plain Dealer" in the figure), one result can be also
considered as one piece of information returned to the user by a
reporter. Besides this ``health care" event, the other two events:
``Shanghai Expo opens/opening\footnote{On April 30 (ET), the
remarkable Shanghai Expo opens, which attracts worldwide attention
for its largest scale in the World Expo history.}" and ``Lakers Jazz
Game 4/four result\footnote{On May 10 (ET), Los Angeles Lakers beats
Utah Jazz in Round 4 of the second round NBA playoffs'10 and then
goes into the semifinals of the playoffs.}" are also considered.
Since the Google News system allows us to add the date constraint
when searching, we use the time constraint to find the reports
between the date of the event and one day after the event to make
the results more relevant. Thus, the date limitations for ``Health
Care", ``Expo" and ``Lakers" are 03/21-03/22, 04/30-04/31,
05/10-05/11 respectively
%\footnote{Since the reporters are located in
%different area of the World thus belonging to different time zone,
%we transfer all of the report times into the corresponding
%representations of ET (North American Eastern Standard Time) time
%zone to check whether they're within the required date range.}
, all are with ET time zone. In addition, we pick up the reports by
obeying the following principles:
\begin{itemize}
  \item The reports generally contain three kinds of sources, i.e., Web Portals, Electronic Newspapers and Blogs.
        We just consider the former two categories which are usually
        thought to have higher reputation than Blogs.
  \item We check the addresses of reporters, and only keep the
        results from reporters with explicit addresses.
  \item If a report is marked by an explanation that it is from the
        event location, then it will be considered as a report from
        the event location no matter what the actual position of the
        reporter is. For example, in the ``health care" event, if a report from Los Angeles Times
        is marked by a one from a employee (journalist) on the White
        House, then the corresponding location for this report
        should be the White House but not the address of the
        magazine office.
  \item Although most reports are original, a few reports actually
        simply copy the contents from
        others. We neglect the un-original ones.
\end{itemize}

\begin{figure}[!t]
\centering
\includegraphics[width=1.8in]{pics/newnew1.eps}
\caption{The distance CDF of different events} \label{fig:new2}
\end{figure}

After the above processing, 63, 88 and 31 reports are chosen for
``Health Care", ``Expo" and ``Lakers". First, from the corresponding
report number, we can generally think that the degree of concern for
the three events is ``Expo" $>$ ``Health Care" $>$ ``Lakers". In
addition, we try to use Fig. \ref{fig:new2} to give some brief
comments about the three events. Because we know the exact location
of the three events: ``Health care" - The White House in Washington,
``Expo" - The Expo Site in Shanghai, ``Lakers" - The Energy
Solutions Arena in Utah, we can calculate the distance between the
reporters and the event locations. The CDF in Fig. \ref{fig:new2}
exhibits some interesting phenomenons. For the ``Health care" event,
22.2\% reporters are within Washington, and 93.7\% reporters are
within the US, which shows this event is a \textbf{National Wide}
event in the US. For the ``Expo" event, only 23.9\% reports are from
China, but more than 75\% reporters show a wide range of world
cities, from London to New York, from Helsinki to Sydney, more than
30 regions are involved. Obviously, this is a \textbf{World Wide}
event. Then, for the ``Lakers" event, all of the reporters are in
the US, but more specifically, nearly 70\% reports are from the
states of two match teams, California and Utah. We can call such
event a \textbf{Local Wide} event.

We believe that the selected events belong to different categories
and are qualified for representing most actual events. We thus use
the reporter distance distribution in the generated dataset to
analyze our proposal in the following sections\footnote{Except for
the real Google News data, we also tried some random data, and the
results are rather similar.}.

\subsection{Setting}
In the evaluation section, we assume at most 4 formats are used.
Also, since the actual distance ($d$) distribution has a very huge
range, we use $\log_{10}d$ to replace $d$ to calculate the
credibility. Recall Eq. \ref{eq:text}, let $\gamma = 1$ and
$h_0=log_{10}100=2$, we have the credibility calculation
\begin{eqnarray} \label{eq:text1}
{c_{i,j}}(S_i,L) = \frac{1}{[\log_{10}{d{{(S_i,L)}}}]^{{\delta _j}}}
\quad &&{2}
\le log_{10}d(S_i,L),{\rm{  }}1 \le j \le 4,\nonumber\\
&&{\delta _1} > {\delta _2} > {\delta _3} > {\delta _4}
\end{eqnarray}
where  thefor both the centralization and the decentralization. It is useful,
since we can use this relationship to estimate the approximate
optimal cost for a certain $k$, or inversely guide to roughly choose
$k$ with expected total cost.

From Fig.\ref{fig:new5b}, it is very obvious that the decentralized
algorithms can greatly reduce the running cost. The running time of
centralized algorithms is several hundred times (sometimes even
several thousand times) as high as that of decentralized ones. For a
specific setting, the running time is decreasing with the increasing
$k$, the reason is as following: Considering Eqs. \ref{eq:dy10} and
\ref{eq:dy} with complexities $O(NRW_{N \times R})$ and $O(NW_N)$,
the larger $k$, the larger $C$, however, the smaller $W$. In other
words, the increasing $k$ actually leads to a decreasing $W$ as well
as a lower computational complexity.


==> renewals2.tex <==

\section{Dynamic Optimization for Systems with Renewals: The General Problem}

Consider a discrete time system with renewals, and let $\{T[1], T[2], T[3], \ldots\}$  represent
the renewal frame durations.  We assume $\{T[k]\}_{k=1}^{\infty}$ is an i.i.d. sequence of positive real numbers, with 
expectation $\expect{T}$.  Every renewal frame $k$, a \emph{random event} $\omega[k]$ is revealed (assumed
to be i.i.d. over frames).  Every frame, the network controller observes the random event $\omega[k]$ and chooses
a \emph{control action} $\alpha[k]$ from a general set of feasible actions $\script{A}_{\omega[k]}$ that possibly
depend on the random event $\omega[k]$.   The random event $\omega[k]$ and the control action $\alpha[k] \in \script{A}_{\omega[k]}$ together determines an $M+1$ dimensional 
vector $\bv{y}[k]$, representing   \emph{network attributes} for frame $k$: 
\[ \bv{y}[k] = (y_0[k], y_1[k], \ldots, y_M[k]) \]
Specifically, each $y_m[k]$ attribute is given by a general function of $\alpha[k]$ and $\omega[k]$: 
\[ y_m[k] = \hat{y}_m(\alpha[k], \omega[k]) \: \: \forall m \in \{0, 1, \ldots, M\} \]
The functions $\hat{y}_m(\alpha[k], \omega[k])$ are arbitrary (possibly non-linear, 
non-convex, discontinuous), and are only assumed
to be bounded. 

Define $\overline{y}_m$ as the time average expectation of the 
attribute $y_m[k]$, averaged over all frames (assuming temporarily that the limit exists): 
\[ \overline{y}_m \defequiv \lim_{k\rightarrow\infty}\frac{1}{K}\sum_{k=1}^K \expect{y_m[k]} \]
The general problem is to find an algorithm for choosing control actions $\alpha[k]$ over time to solve: 
\begin{eqnarray} 
\mbox{Minimize:} && \overline{y}_0 \\
\mbox{Subject to:} &1)& \overline{y}_m \leq 0 \: \: \forall m \in \{1, 2, \ldots, M\} \\
&2)& \alpha[k] \in \script{A}_{\omega[k]} \mbox{ $\forall$ frames $k \in \{1, 2, \ldots\}$}  
\end{eqnarray} 

The solution to the general problem is given in terms of a positive parameter $V$, which affects a peformance tradeoff. 
Specifically, for each of the $M$ 
time average inequality constraints $\overline{y}_m \leq 0$, define a \emph{virtual queue} $Z_m[k]$ with $Z_m[0] = 0$, and 
with frame update equation: 
\begin{equation} \label{eq:z-update} 
 Z_m[k+1] = \max[Z_m[k] + y_m[k], 0] 
 \end{equation} 
 Then every frame $k$, observe the value of $\omega[k]$ and perform the following actions: 
 \begin{itemize} 
 \item Choose $\alpha[k]$ to solve: 
 \begin{eqnarray*}
 \mbox{Min:} & V\hat{y}_0(\alpha[k], \omega[k]) + \sum_{m=1}^MZ_m[k]\hat{y}_m(\alpha[k], \omega[k]) \\
 \mbox{Subj. to:} & \alpha[k] \in \script{A}_{\omega[k]} 
 \end{eqnarray*}
 \item Update the virtual queues $Z_m[k]$ according to (\ref{eq:z-update}), using the values $y_m[k] = \hat{y}_m(\alpha[k], \omega[k])$ determined from the above minimization. 
 \end{itemize} 
 
 Assuming the problem is feasible (so that it is possible to meet the time average inequality constraints), this algorithm
 will \emph{also} meet all of these constraints, and will achieve a time average value $\overline{y}_0$ that is within $O(1/V)$
 of the optimum.   Typically, the $V$ parameter also affects the average size of the virtual queues (these can be shown to 
 be $O(V)$, which directly affects the \emph{convergence time} needed for the time averages to be close to their limiting
 values.  The theory is developed in \cite{now}\cite{neely-energy-it}\cite{neely-thesis}, with minor notational adjustments
 needed to change the timeslot averages there to frame-averages here. 
 
  
 \section{Application to Power-Aware Credibility Problems} 
 
 Consider now the following problem:  There are $N$ wireless devices.  Events occur according to a renewal 
 process with i.i.d. inter-renewal times $\{T[1], T[2], \ldots\}$ with finite mean $\expect{T}$ (in units of time, such as seconds). 
At the beginning of every renewal frame $k$, a random vector $\bv{A}[k] = (A_1[k], \ldots, A_N[k])$ of information arrives, 
together with a vector $\bv{M}[k] = (M_1[k], \ldots, M_N[k])$ of \emph{meta-data}. The $A_n[k]$ value represents data 
that is sensed at device $n$ on frame $k$, and the meta-data $M_n[k]$ represents additional information concerning 
the importance or credibility of this data, as well as its ``compression'' properties.  In particular, this data must be communicated
using one of multiple transmission modes (such as voice or video), and the meta-data can suggest how the information will
be distorted in each of the different modes.  Let $\omega[k] = (\bv{A}[k]; \bv{M}[k])$ represent the overall random event associated
with frame $k$.  

Let $\alpha[k] = (\alpha_1[k], \ldots, \alpha_N[k])$ be a vector of modes for transmission, where $\alpha_n[k]$ represents
the transmission mode of device $n$ on frame $k$, chosen within some abstract set $\script{A}_{\omega[k]}$. For example,
this set might be the set that allows each entry $\alpha_n[k]$ to be chosen from one of 3 options:  no attempted transmission, 
transmission with text mode, transmission with video mode.   The set might also constrain the decisions to meet some minimum
required credibility level for each frame, and/or might constrain the total sum of 

Let $\bv{p}[k] = (p_1[k], \ldots, p_N[k])$ represent the vector of  \emph{power expenditures} associated with each device
on frame $k$, being a general function of the decision: 
\[ p_n[k] = \hat{p}_n(\alpha_n[k], \omega[k]) \]
If power is not an issue, these can represent other general costs. 
Let $c[k]$ be an overall ``credibility value function'' associated with decisions: 
\[ c[k] \defequiv \hat{c}(\alpha[k], \omega[k]) \]
Let $b[k]$ represent the total bandwidth required to fulfill the chosen actions on frame $k$: 
\[ b[k] \defequiv \hat{b}(\alpha[k], \omega[k]) \]
The goal is to maximize a time average credibility, subject to time average power constraints, and to additional 
per-frame credibility and bandwidth constraints: 
\begin{eqnarray*}
\mbox{Maximize:} && \overline{c} \\
\mbox{Subject to:} &1)& \frac{\overline{p}_n}{\expect{T}} \leq P_n^{av}  \: \: \forall n \in \{1, \ldots, N\} \\
&2)& \hat{c}(\alpha[k], \omega[k]) \geq c_{min} \: \: \forall k \in \{1, 2, \ldots \} \\
&3)& \hat{b}(\alpha[k], \omega[k]) \leq b_{max} \: \: \forall k \in \{1, 2, \ldots \} \\
&3)& \alpha[k] \in \script{A}_{\omega[k]} \: \: \forall k \in \{1, 2, \ldots \} 
\end{eqnarray*}
where $c_{min}$ is a given constant that represents a desired minimum credibility level per frame, 
$b_{max}$ is a maximum bandwidth constraint per frame, 
and $P_n^{av}$ for $n \in \{1, \ldots, N\}$ are given constants that represent average power constraints 
for each wireless device.   Note that these power constraints are in units of power-per-unit-time, rather than
power-per-frame.  Hence, we must normalize $\overline{p}_n$ by dividing it by the (potentially unknown) average
frame duration $\expect{T}$.  This problem can be transformed into the general framework by defining
$y_n[k] \defequiv p_n[k] - P_n^{av}T[k]$, and noting that $\overline{y}_n \leq 0$ corresponds to 
$\overline{p}_n/\expect{T} \leq P_n^{av}$.   We can treat this problem of maximizing $\overline{c}$ by using
$y_0[k] \defequiv -c[k]$.  The full solution is given by defining 
virtual queues $Z_n[k]$ (for $n \in \{1, \ldots, N\}$)  as follows: 
\begin{eqnarray} 
Z_n[k+1] &=& \max[Z_n[k] + p_n[k] - P_n^{av}T[k], 0]  \label{eq:z-update-p1} 
\end{eqnarray} 
The virtual queues $Z_n[k]$ are designed to enforce the $\overline{p}_n/\expect{T} \leq P_n^{av}$ constraint.

The solution is then given as follows: Every frame $k$, observe $\omega[k]$.  Then: 
\begin{itemize} 
\item Take an action $\alpha[k]$ that solves: 
\begin{eqnarray*}
\mbox{Maximize:} & V\hat{c}(\alpha[k], \omega[k]) - \sum_{n=1}^N Z_n[k]\hat{p}_n(\alpha[k], \omega[k]) \\
\mbox{Subject to:} & \alpha[k] \in \script{A}_{\omega[k]} \\
& \hat{c}(\alpha[k], \omega[k]) \geq c_{min} \\
& \hat{b}(\alpha[k], \omega[k]) \leq b_{max} 
\end{eqnarray*}
\item Update virtual queues $Z_n[k]$ according to (\ref{eq:z-update-p1}). 
\end{itemize} 

Assuming feasibility, this algorithm again achieves a time average $\overline{c}$ that is within $O(1/V)$ of optimal. 
All desired time average power constraints are met, with average virtual queue size $O(V)$ (which means the 
average ``lag'' over which the power constraints are violated over any interval is $O(V)$, regarless of the interval size). 

\subsection{On Knapsack Problems} 

Let us temporarily assume $c_{min} = 0$, so that the $\hat{c}(\alpha[k], \omega[k])$ constraint is removed. Let us
further assume that: 
\[ \hat{b}(\alpha[k], \omega[k]) = \sum_{n=1}^N \hat{b}_n(\alpha_n[k], \omega_n[k]) \]
\[ \hat{c}(\alpha[k], \omega[k]) = \sum_{n=1}^N \hat{c}_n(\alpha_n[k], \omega_n[k]) \]
where $\alpha_n[k]$ and $\omega_n[k]$ are control actions and events local to device $n$.  Then the 
solution above reduces to a basic knapsack problem every slot, using virtual queue weights to keep track
of the running averages of power expenditure. 

However, one can relax the constraint  $\hat{b}(\alpha[k], \omega[k]) \leq b_{max}$, which restricts the total bits
to $b_{max}$ per frame, to an \emph{average} bandwidth constraint of the form: 
\[ \overline{b} \leq b_{max} \]
where: 
\[ \overline{b} \defequiv \lim_{k\rightarrow\infty}\frac{1}{K} \sum_{k=1}^K \expect{b[k]} \]
This version of the problem gets around the complex knapsack operation, and reduces to an algorithm that makes
simple (and distributed) actions at each node.  That is because the variables associated with each device
occur in separate terms of the function that needs to be minimized on each slot of the algorithm.  
We can in fact define an actual queue of bits, and we can then 
show that this actual queue of bits has average size $O(V)$, which also affects the average delay. 
This gives an $O(1/V)$ distance to the optimal time average credibility, with $O(V)$ average delay. 


% ------------------------------------------------------------------------
%GATHER{Xbib.bib}   % For Gather Purpose Only
%GATHER{Paper.bbl}  % For Gather Purpose Only
%\bibliographystyle{unsrt}
%\bibliographystyle{plain}
%\bibliography{../../latex-mit/bibliography/refs}
%\end{document}
% ------------------------------------------------------------------------









==> renewals2_bin.tex <==

\section{The Renewals Problem}
\label{sec:renewals}

In the previous section, we discussed a one-shot problem: that of
optimizing a single event.
%
We now consider a formulation which considers a sequence of event
arrivals as \emph{renewals}\footnote{The assumption here is that
  events do not overlap in time.}.
%
In this setting, we consider a stochastic variant of \minC: instead of
minimizing cost for a single event, we minimize the average cost
asymptotically.
%
Interestingly, this formulation yields nice properties: it is provably
near-optimal, and, for additive corroboration functions, \emph{decisions
  can be made in a decentralized fashion} (i.e., individual reporters
can make uncoordinated decisions, without any intervention from the
swarm director).
%
We start by solving the general problem of dynamic optimization for
systems with renewals using Lyapunov analysis, then show how it
applies in our setting, and conclude with a discussion of the
relationship to online knapsack problems.

\subsection{The  General Problem}
\label{sec:renewals:general}

Consider a discrete time system with renewals, and let $\{T[1], T[2],
T[3], \ldots\}$ represent the renewal frame durations.
%
We assume $\{T[k]\}_{k=1}^{\infty}$ is an i.i.d.\ sequence of positive
real numbers, with expectation $\expect{T}$.
%
Every renewal frame $k$, a \emph{random event} $\omega[k]$ is revealed
(assumed to be i.i.d.\ over frames).
%
In every frame, the director observes the random event $\omega[k]$ and
chooses a \emph{control action} $\alpha[k]$ from a general set of
feasible actions $\script{A}_{\omega[k]}$ that possibly depend on the
random event $\omega[k]$.
%
The random event $\omega[k]$ and the control action $\alpha[k] \in
\script{A}_{\omega[k]}$ together determines an $M+1$ dimensional
vector $\bv{y}[k]$, representing \emph{network attributes} for frame
$k$:
%
\[ \bv{y}[k] = (y_0[k], y_1[k], \ldots, y_M[k]) \]
%
Specifically, each $y_m[k]$ attribute is given by a general function
of $\alpha[k]$ and $\omega[k]$:
%
\[ y_m[k] = \hat{y}_m(\alpha[k], \omega[k]) \: \: \forall m \in \{0, 1, \ldots, M\} \]
%
The functions $\hat{y}_m(\alpha[k], \omega[k])$ are arbitrary
(possibly non-linear, non-convex, discontinuous), and are only assumed
to be bounded.

Define $\overline{y}_m$ as the time average expectation of the
attribute $y_m[k]$, averaged over all frames (assuming temporarily
that the limit exists):
%
\[ \overline{y}_m \defequiv \lim_{k\rightarrow\infty}\frac{1}{K}\sum_{k=1}^K \expect{y_m[k]} \]
%
The general problem is to find an algorithm for choosing control
actions $\alpha[k]$ over time to solve:
\begin{eqnarray}
\mbox{Minimize:} && \overline{y}_0 \\
\mbox{Subject to:} &1)& \overline{y}_m \leq 0 \: \: \forall m \in \{1, 2, \ldots, M\} \\
&2)& \alpha[k] \in \script{A}_{\omega[k]} \mbox{ $\forall$ frames $k \in \{1, 2, \ldots\}$}
\end{eqnarray}

The solution to the general problem is given in terms of a positive
parameter $V$, which affects a peformance tradeoff.
%
Specifically, for each of the $M$ time average inequality constraints
$\overline{y}_m \leq 0$, define a \emph{virtual queue} $Z_m[k]$ with
$Z_m[0] = 0$, and with frame update equation:
%
\begin{equation} \label{eq:z-update}
 Z_m[k+1] = \max[Z_m[k] + y_m[k], 0]
 \end{equation}
%
Then every frame $k$, observe the value of $\omega[k]$ and perform
the following actions:
 \begin{itemize}
 \item Choose $\alpha[k]$ to solve:
 \begin{eqnarray*}
 \mbox{Min:} & V\hat{y}_0(\alpha[k], \omega[k]) + \sum_{m=1}^MZ_m[k]\hat{y}_m(\alpha[k], \omega[k]) \\
 \mbox{Subj. to:} & \alpha[k] \in \script{A}_{\omega[k]}
 \end{eqnarray*}
 \item Update the virtual queues $Z_m[k]$ according to (\ref{eq:z-update}), using the values $y_m[k] = \hat{y}_m(\alpha[k], \omega[k])$ determined from the above minimization.
 \end{itemize}

Assuming the problem is feasible (so that it is possible to meet the
time average inequality constraints), this algorithm will \emph{also}
meet all of these constraints, and will achieve a time average value
$\overline{y}_0$ that is within $O(1/V)$ of the optimum.
%
Typically, the $V$ parameter also affects the average size of the
virtual queues (these can be shown to be $O(V)$, which directly
affects the \emph{convergence time} needed for the time averages to be
close to their limiting values.
%
The proofs of these claims follow the theory is developed
in~\cite{now,neely-energy-it,neely-thesis}, with minor notational
adjustments needed to change the timeslot averages there to
frame-averages here.
%
We omit these proofs for brevity.

\subsection{Formulating Corroboration Pull as a Dynamic Optimization
  Problem}
\label{sec:renewals:corrob}

Consider now the following dynamic problem our corroboration problem
with $N$ reporters.
%
Events occur according to a renewal process with i.i.d.\
inter-renewal times $\{T[1], T[2], \ldots\}$ with finite mean
$\expect{T}$ (in units of time, such as seconds).
%
At the beginning of every renewal frame $k$, a random vector
$\bv{A}[k] = (A_1[k], \ldots, A_N[k])$ of information arrives,
together with a vector $\bv{M}[k] = (M_1[k], \ldots, M_N[k])$ of
\emph{meta-data}.
%
$A_n[k]$ value represents data that is observed by reporter $n$ on
frame $k$, and the meta-data $M_n[k]$ represents the importance or
credibility of this data.
%
In particular, this data must be reported to the director using one of
multiple report formats (such as text, audio or video), and the
meta-data can suggest how the information will be distorted in each of
the different formats.
%
Let $\omega[k] = (\bv{A}[k]; \bv{M}[k])$ represent the overall random
event associated with frame $k$.
%

Let $\alpha[k] = (\alpha_1[k], \ldots, \alpha_N[k])$ be a vector of
reports for reporting, where $\alpha_n[k]$ represents the employed
report format of reporter $n$ on frame $k$, chosen within some
abstract format set $\script{A}_{\omega[k]}$.
%
For example, this set might be the set that allows each entry
$\alpha_n[k]$ to be chosen from one of 3 options: no attempted report,
reporting with text mode, reporting with video mode.
%
The set might also constrain the decisions to meet some minimum
required credibility level (target) for each frame, and/or might
constrain the total sum of bandwidth.
%

In the previous sections, we define "cost" as the general cost
including various resource consumptions, and here, we would like to
further refine "cost" to two aspects: the \emph{power expenditure} and
the \emph{bandwidth consumption}.
%
Such refined definition can help us obtain a very general framework
about the credibility renewal problems.
%

Let $\bv{p}[k] = (p_1[k], \ldots, p_N[k])$ represent the vector of
\emph{power expenditures} associated with each reporter on frame
$k$, being a general function of the decision:
\[ p_n[k] = \hat{p}_n(\alpha_n[k], \omega[k]) \] Let $c[k]$ be an
overall ``credibility value function'' (the function can be either in
the form of Eq.\ref{eq:text}, Eq.\ref{eq:cnoise} or some others)
associated with decisions:
%
\[ c[k] \defequiv \hat{c}(\alpha[k], \omega[k]) \]
%
Let $b[k]$ represent the total bandwidth required to fulfill the
chosen actions on frame $k$:
%
\[ b[k] \defequiv \hat{b}(\alpha[k], \omega[k]) \]
%
The goal is to maximize a time average credibility, subject to time
average power constraints, and to additional per-frame credibility and
bandwidth constraints:
\begin{eqnarray*}
\mbox{Maximize:} && \overline{c} \\
\mbox{Subject to:} &1)& \frac{\overline{p}_n}{\expect{T}} \leq P_n^{av}  \: \: \forall n \in \{1, \ldots, N\} \\
&2)& \hat{c}(\alpha[k], \omega[k]) \geq c_{min} \: \: \forall k \in \{1, 2, \ldots \} \\
&3)& \hat{b}(\alpha[k], \omega[k]) \leq b_{max} \: \: \forall k \in \{1, 2, \ldots \} \\
&3)& \alpha[k] \in \script{A}_{\omega[k]} \: \: \forall k \in \{1, 2, \ldots \}
\end{eqnarray*} where $c_{min}$ is a given constant that represents a
desired minimum credibility level per frame, $b_{max}$ is a maximum
bandwidth constraint per frame, and $P_n^{av}$ for $n \in \{1, \ldots,
N\}$ are given constants that represent average power constraints for
each reporter.
%
Note that these power constraints are in units of power-per-unit-time,
rather than power-per-frame.
%
Hence, we must normalize $\overline{p}_n$ by dividing it by the
(potentially unknown) average frame duration $\expect{T}$.
%
This problem can be transformed into the general framework by defining
$y_n[k] \defequiv p_n[k] - P_n^{av}T[k]$, and noting that
$\overline{y}_n \leq 0$ corresponds to $\overline{p}_n/\expect{T} \leq
P_n^{av}$.
%
We can treat this problem of maximizing $\overline{c}$ by using
$y_0[k] \defequiv -c[k]$.
%
The full solution is given by defining virtual queues $Z_n[k]$ (for $n
\in \{1, \ldots, N\}$) as follows:
%
\begin{eqnarray}
Z_n[k+1] &=& \max[Z_n[k] + p_n[k] - P_n^{av}T[k], 0]  \label{eq:z-update-p1}
\end{eqnarray}
The virtual queues $Z_n[k]$ are designed to enforce the
$\overline{p}_n/\expect{T} \leq P_n^{av}$ constraint.

The solution is then given as follows: Every frame $k$, observe
$\omega[k]$.  Then:
\begin{itemize}
\item Take an action $\alpha[k]$ that solves:
\begin{eqnarray*}
\mbox{Maximize:} & V\hat{c}(\alpha[k], \omega[k]) - \sum_{n=1}^N Z_n[k]\hat{p}_n(\alpha[k], \omega[k]) \\
\mbox{Subject to:} & \alpha[k] \in \script{A}_{\omega[k]} \\
& \hat{c}(\alpha[k], \omega[k]) \geq c_{min} \\
& \hat{b}(\alpha[k], \omega[k]) \leq b_{max}
\end{eqnarray*}
\item Update virtual queues $Z_n[k]$ according to (\ref{eq:z-update-p1}).
\end{itemize}

Assuming feasibility, this algorithm again achieves a time average
$\overline{c}$ that is within $O(1/V)$ of optimal.
%
All desired time average power constraints are met, with average
virtual queue size $O(V)$ (which means the average ``lag'' over which
the power constraints are violated over any interval is $O(V)$,
regarless of the interval size).
%

\subsection{On Knapsack Problems}
\label{sec:renewals:knapsack}

Once again, we could try to associate the discussed problems with the
Knapsack Problems.
%
Let us temporarily assume $c_{min} = 0$, so that the
$\hat{c}(\alpha[k], \omega[k])$ constraint is removed.
%
Let us further assume that:
%
\[ \hat{b}(\alpha[k], \omega[k]) = \sum_{n=1}^N \hat{b}_n(\alpha_n[k], \omega_n[k]) \]
\[ \hat{c}(\alpha[k], \omega[k]) = \sum_{n=1}^N \hat{c}_n(\alpha_n[k],
\omega_n[k]) \] where $\alpha_n[k]$ and $\omega_n[k]$ are control
actions and events local to reporter $n$.
%
Then the solution above reduces to a basic knapsack problem every
slot, using virtual queue weights to keep track of the running
averages of power expenditure.
%

However, one can relax the constraint $\hat{b}(\alpha[k], \omega[k])
\leq b_{max}$, which restricts the total bits to $b_{max}$ per frame,
to an \emph{average} bandwidth constraint of the form:
%
\[ \overline{b} \leq b_{max} \]
where:
\[ \overline{b} \defequiv \lim_{k\rightarrow\infty}\frac{1}{K}
\sum_{k=1}^K \expect{b[k]} \]
%
This version of the problem gets around the complex knapsack
operation, and reduces to an algorithm that makes simple (and
distributed) actions at each reporter.
%
That is because the variables associated with each reporter occur in
separate terms of the function that needs to be minimized on each slot
of the algorithm.
%
We can in fact define an actual queue of bits, and we can then show
that this actual queue of bits has average size $O(V)$, which also
affects the average delay.
%
This gives an $O(1/V)$ distance to the optimal time average
credibility, with $O(V)$ average delay.
%


% ------------------------------------------------------------------------
%GATHER{Xbib.bib}   % For Gather Purpose Only
%GATHER{Paper.bbl}  % For Gather Purpose Only
%\bibliographystyle{unsrt}
%\bibliographystyle{plain}
%\bibliography{../../latex-mit/bibliography/refs}
%\end{document}
% ------------------------------------------------------------------------


==> rule.tex <==
\section{Rule-based one shot problem}
\label{sec:rule}


\subsection{Framework of rule-based credibility}
As discussed in Section \ref{sec:defrule}, the rule-based
credibility actually acts as a boolean function whose input and
output are a set of reports and a boolean conclusion (credible or
incredible), respectively.

We implement such a boolean function by defining a series of rules.
For each report format $i$, we create $q_i$ categories, and each
category corresponds to a distance range. Note that the range should
be considered with the applicable threshold discussed in Section
\ref{sec:stra} integrally. Then, each rule contains
$\sum\nolimits_{i = 1}^n {{q_i}}$ non-negative integers for each of
the $\sum\nolimits_{i = 1}^n {{q_i}}$ categories, and these integers
also define the required report number of the corresponding
categories in a rule. Actually, the category based distance division
further refines the format based one, thus offers more flexible in
defining the rules.

\begin{table*}
\centering \scriptsize \caption{An example of credibility rules}
\setlength\doublerulesep{0pt}
\setlength{\baselineskip}{1.5\baselineskip}
\begin{tabular}[h]{||c|c|c|c|c|c|c|c|c|c|c|c|c|c||}
\hline \hline
\multirow{2}{*}{Rules}& \multirow{2}{*}{Cost} & \multicolumn{4}{c|}{format\_1 (Text)} & \multicolumn{4}{c|}{format\_2 (low quality video)} & \multicolumn{4}{c||}{format\_3 (high quality video)}\\
\cline{3-14}
&& $< 30m$ & $\#got$ & $30m-70m$ & $\#got$ & $< 90m$ & $\#got$ & $90m-120m$ & $\#got$& $< 140m$ & $\#obtained$ & $140m-170m$ & $\#obtained$\\
\hline
rule5 &12& 0 & \bf{(+10)} & 0 &  & 0 & \bf{(+1)} & 0 &  & 1 & \bf{1} & 1 & \bf{(-1)}\\
\hline
rule1 &15& 15 & \bf{10 (-5)} & 0 &  & 0 & \bf{(+1)} & 0 &  & 0 & \bf{(+1)} & 0 &  \\
\hline
rule4 &18& 0 & \bf{(+10)} & 0 &  & 0 &  & 3 & \bf{1 (-2)} & 0 &  & 1 & \bf{1}\\
\hline
rule2 &20& 0 &  & 20 & \bf{10 (-10)} & 0 & \bf{(+1)} & 0 &  & 0 & \bf{(+1)} & 0 &  \\
\hline
rule3 &25& 5 & \bf{5} & 6 & \bf{5 (-1)} & 1 & \bf{1} & 0 &  & 1 & \bf{1} & 0 & \\
\hline \hline
\end{tabular}
\label{tab:haha}
\end{table*}

An example is shown in Table \ref{tab:haha}. In this example, we
have three report formats -- text, low quality video and high
quality video with the distance thresholds $h_1 = 30m$, $h_2 = 70m$
and $h_3 = 120m$, respectively. For each format, we have two
categories distinguished by the range. Five rules are defined as
shown in the table. Also, we sort the five rules in ascending order
of cost (note that we can estimate the total cost of each rule
previously). Therefore, the destination station can maintain this
table and tries to fill in this table during receiving reports. As
long as all of the positive integers of one rule (column) have been
achieved, the destination would think the report set is credible, or
it would adjust the strategy of some reporters to try to achieve a
certain rule. Furthermore, if none rule could be fulfilled even
after adjusting, the destination would think the rules based
credibility could not be obtained with the existing reporter
deployment. \textbf{Note that for the categories in a same format, a
high level category report can be also used to fill in a grid of a
low level category.} For example, if the destination receives a text
report with a $25m$ distance to the event location, then this report
can be used to fill in either the ``$<30m$" grid or the ``$30m-70m$"
grid according to the necessary. For example, in rule1, the report
would be used to fill in the ``$<30m$" grid, while it should be used
to fill in the ``$30m-70m$" grid in rule2.

Now, supposing that 15 reporters are monitoring an event and choose
their preference report formats according to the relationship
between the distance and the strategy introduced in Section
\ref{sec:stra}, and these preference reports contain ten ``$<30m$"
text reports, one ``$70m-90m$" low quality video report, one
``$120m-140m$" high quality video report and three ``$>170m$" high
quality video reports. Then, the three ``$>170m$" text reports are
of no use since no rule needs them, while other reports can be used
to fill in the rule grids as shown by the unsigned bold numbers.

\subsection{Mechanism Design}


Still consider Table \ref{tab:haha}, it is found that with the
preference reporter configuration, no rules is satisfied. In order
to try to achieve at least one rule, the destination can try to
adjust the report strategies of some reporters.

By marking the redundancy or deficiency number in each report
categories with signed bold numbers, we can get the following
observation: If one rule has not been satisfied yet, then it can be
satisfied by adjusting the report strategies of some reporters as
long as - by going through this rule from left to right in Table
\ref{tab:haha}, the sum of the signed bold number should never go
negative. The reason why we goes through from left to right is
because the applicable distance ranges of report categories are
increasing from left to right. The consideration that -
\textbf{format\_$i$ reporter can be switched to a format\_$j
(i<j\leq n)$ reporter and the new format\_$j$ reports after
switching is qualified to fill in any category grid associated with
format\_$j$} - is just similar as the discussion about Algorithm
\ref{al:ad} in Section \ref{sec:numopt}. So, it is obvious that in
Table \ref{tab:haha}, rule1, rule2 and rule3 still cannot be
fulfilled by adjusting since the sums of the signed numbers go to
negative with -5, -10 and -1, but rule4 or rule5 can be fulfilled by
switching two or one format\_1 reporters to two format\_2 reporters
or one format\_3 reporter respectively because the sums of the
signed numbers are kept non-negative all the time from left to
right. In addition, if going on to consider the cost of each rule,
we would try to achieve rule5 rather than rule4 through the
adjustment due to the relative less cost of rule5. Also, since rule5
only needs two format\_3 reporters, we could actually only enable
the two reporters but disable others to reduce the total cost.

Thus, our mechanism for rules based credibility is trying to find
the satisfied minimum cost rule or trying to achieve the minimum
cost rule among all of the potential satisfiable rules by adjusting
the behaviors of reporters (change their preference report formats).
The specific algorithm is shown in Algorithm \ref{al:op3}. It is
easy to obtain the time complexity for each decision interval is
$O$(the scale of table).

\begin{algorithm}
  \caption{Fulfill the rules based credibility in each decision interval}
  \label{al:op3}
  \begin{algorithmic}[1]
    \STATE like Table \ref{tab:haha}, create and sort a table contains the cost and requirements of all the rules;
    \STATE the preference format set $F = \{f_1, f_2,\ldots,
    f_m \}$
    \FOR{each rule$\_i$}
    \STATE fill in the $\#got$ fields of each rule using $F$;
    \IF{rule$\_i$ is satisfied}
    \RETURN credible;
    \ENDIF
    \ENDFOR
    \FOR{each rule$\_i$}
    \IF{sum of signed numbers $\geq 0$}
    \STATE adjust the behaviors of reporters (change their preference report formats) to achieve rule$\_i$
    \RETURN credible;
    \ENDIF
    \ENDFOR
    \RETURN incredible;
  \end{algorithmic}
\end{algorithm}

